Automated speech- and text-based classification of neuropsychiatric conditions in a multidiagnostic setting

Speech patterns have been identified as potential diagnostic markers for neuropsychiatric conditions. However, most studies only compare a single clinical group to healthy controls, whereas clinical practice often requires differentiating between multiple potential diagnoses (multiclass settings). To address this, we assembled a dataset of repeated recordings from 420 participants (67 with major depressive disorder, 106 with schizophrenia and 46 with autism, as well as matched controls), and tested the performance of a range of conventional machine learning models and advanced Transformer models on both binary and multiclass classification, based on voice and text features. While binary models performed comparably to previous research (F1 scores between 0.54-0.75 for autism spectrum disorder, ASD; 0.67-0.92 for major depressive disorder, MDD; and 0.71-0.83 for schizophrenia); when differentiating between multiple diagnostic groups performance decreased markedly (F1 scores between 0.35-0.44 for ASD, 0.57-0.75 for MDD, 0.15-0.66 for schizophrenia, and 0.38-0.52 macro F1). Combining voice and text-based models yielded increased performance, suggesting that they capture complementary diagnostic information. Our results indicate that models trained on binary classification may learn to rely on markers of generic differences between clinical and non-clinical populations, or markers of clinical features that overlap across conditions, rather than identifying markers specific to individual conditions. We provide recommendations for future research in the field, suggesting increased focus on developing larger transdiagnostic datasets that include more fine-grained clinical features, and that can support the development of models that better capture the complexity of neuropsychiatric conditions and naturalistic diagnostic assessment.

==> Examples/ex_initial_on_section.tex <==
\paragraph{}{\footnotesize KCE \& XXX \newline}

\noindent
%text

==> Examples/ex_qoutes.tex <==
\subsection{Example of anonymization} \label{app:example}
A sample article from the Danish news media, DR.
\begin{quote}
I Herlev kan de blandt andet se frem til 35 nyopslåede stillinger.
I en række kommuner har byrådene selv fundet penge til at sikre minimumsnormeringer. (Foto: liselotte sabroe © Scanpix) AF ANN SOPHIE LIER RASMUSSEN 13. NOV. 2019 KL. 15.01 | OPDATERET 13. NOV. 2019 KL. 18.55 Målet med minimumsnormeringen er at sikre, at der højst er tre børn pr. voksen i vuggestuerne og seks børn pr. voksen i børnehaverne. 
\end{quote}

\noindent The sample anonymized using DeepAnon using DaNLP and the rule based approach.
\begin{quote}
I [<B-LOC>] kan de blandt andet se frem til [<NUMBER>] nyopslåede stillinger. I en række kommuner har byrådene selv fundet penge til at sikre minimumsnormeringer . (Foto: liselotte sabroe © Scanpix) AF [<B-PER>] [<I-PER>] [<I-PER>] [<I-PER>] 13. NOV. [<NUMBER>] KL. [<NUMBER>] | OPDATERET 13. NOV. [<NUMBER>] KL. [<NUMBER>] LÆS OP Målet med  minimumsnormeringen er at sikre , at der højst er [<NUMBER>] børn pr. voksen i vuggestuerne og [<NUMBER>] børn pr. voksen i børnehaverne .
\end{quote}

\noindent The ideal anonymization of the sample.
\begin{quote}
I <LOC-1> kan de blandt andet se frem til <NUM-1> nyopslåede stillinger. I en række kommuner har byrådene selv fundet til at sikre minimumsnormeringer. (Fote: <PERS-1> (C) <ORG-2>) AF <PERS-2> <DATE-1> <TIME-1> OPDATERET <DATE-1> <TIME-2> Målet med minimumsnormering er at sikre, at der højst er <NUM-2> børn pr. voksen i vuggestuerne og <NUM-3> børn pr. voksen i børnehaverne.
\end{quote}

\noindent The ideal anonymization of the with tags replaced. Note that in general the meaning of the text is maintained.
\begin{quote}
I Randers kan de blandt andet se frem til 72 nyopslåede stillinger. I en række kommuner har byrådene selv fundet til at sikre minimumsnormeringer. (Foto: Marlene Johnsen (C) Novo Nordisk) AF Toke Dyrhauge 3. December KL. 12.45 OPDATERET 3. December 18.45 Målet med minimumsnormering er at sikre, at der højst er 9 børn pr. voksen i vuggestuerne og 2 børn pr. voksen i børnehaverne.
\end{quote}

==> Examples/ex_table.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c|p{10cm}|} 
\hline
\multicolumn{2}{|c|}{"Charlie hasn't been seen in days. If you see him please call 11-22-33-44."} \\
\hline
\hline
daNLP       & ['Charlie', 'hasn't', 'been', 'seen', 'in', 'days.', 'If', 'you',   'see', 'him', 'please', 'call', '11-22-33-44.'] \\ 
\hline
polyglot    & ['Charlie', 'hasn't', 'been', 'seen', 'in', 'days', '.', 'If', 'you', 'see', 'him', 'please', 'call', '11', '-', '22', '-', '33','-', '44', '.'] \\ 
\hline
stanfordNLP & ['Charlie', 'hasn't', 'been', 'seen', 'in', 'days', '.', 'If', 'you', 'see', 'him', 'please', 'call', '11-22-33-44', '.'] \\ 
\hline
\end{tabular}
\caption{Resulting tokenization of using Danish NLP frameworks}
\label{token_table}
\end{table}

==> Examples/ex_table2.tex <==
% kig på layout sammen, det er ret nemt at ændre placering

\begin{comment}
%%%
%UDEN NA row og columns
%%%
\begin{table}[h]
    \caption{Confusion matrices for the models. Note that the columns do not necessarily sum to the same number in the different tables since DaNLP and Polyglot use different tokenizers.}    
    \label{tab:conf_mat}
    \begin{subtable}[h]{\textwidth}
        \centering
        \begin{tabular}{lrrr}
        \toprule
          & LOC & ORG & PERS\\
        \midrule
        LOC & 403 & 27 & 4\\
        ORG & 629 & 344 & 26\\
        PERS & 20 & 68 & 871\\
        \bottomrule
        \end{tabular}
       \caption{Danlp + Rule based}
       \label{tab:conf_d+r}
    \end{subtable}
    %\hspace*{\fill}
    \newline
    \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{lrrr}
        \toprule
        & LOC & ORG & PERS\\
        \midrule
        LOC & 403 & 27 & 4\\
        ORG & 629 & 344 & 26\\
        PERS & 20 & 66 & 819\\
        \bottomrule
        \end{tabular}
        \caption{DaNLP}
        \label{tab:conf_d}
     \end{subtable}
     \hspace*{\fill}
     \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{lrrr}
        \toprule
          & LOC & ORG & PERS\\
        \midrule
        LOC & 605 & 18 & 3\\
        ORG & 141 & 123 & 8\\
        PERS & 14 & 55 & 826\\
        \bottomrule
        \end{tabular}
        \caption{Polyglot}
        \label{tab:conf_p}
     \end{subtable}
     \newline
    \vspace*{0.5 cm}
    \newline
     %\hspace*{\fill}
     \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{lrrr}
        \toprule
        & LOC & ORG & PERS\\
        \midrule
        LOC & 495 & 34 & 14\\
        ORG & 657 & 413 & 26\\
        PERS & 25 & 103 & 969\\
        \bottomrule
        \end{tabular}
        \caption{DaNLP + Polyglot}
        \label{tab:conf_d+p}
    \end{subtable}
    \hspace*{\fill}
    \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{lrrr}
        \toprule
        & LOC & ORG & PERS\\
        \midrule
        LOC & 722 & 40 & 13\\
        ORG & 428 & 402 & 20\\
        PERS & 27 & 108 & 962\\
        \bottomrule
        \end{tabular}
        \caption{Polyglot + DaNLP}
        \label{tab:conf_p+d}
    \end{subtable}

\end{table}
\end{comment}

\begin{table}[h]
    \caption{Confusion matrices for the models. Note that the columns do not necessarily sum to the same number in the different tables since DaNLP and Polyglot use different tokenizers.}    
    \label{tab:conf_mat}
    \begin{subtable}[h]{\textwidth}
        \centering
        \begin{tabular}{lrrrr}
        \toprule
        & LOC & ORG & PERS & NA\\
        \midrule
        LOC & 403 & 27 & 4 & 104\\
        ORG & 629 & 344 & 26 & 2662\\
        PERS & 20 & 68 & 871 & 254\\
        NA & 317 & 385 & 360 & 56714\\
        \bottomrule
        \end{tabular}
       \caption{Danlp + Rule based}
       \label{tab:conf_d+r}
    \end{subtable}
    %\hspace*{\fill}
    \newline
    \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{lrrrr}
        \toprule
          & LOC & ORG & PERS & NA\\
        \midrule
        LOC & 403 & 27 & 4 & 104\\
        ORG & 629 & 344 & 26 & 2661\\
        PERS & 20 & 66 & 819 & 169\\
        NA & 352 & 386 & 412 & 58382\\
        \bottomrule
        \end{tabular}
        \caption{DaNLP}
        \label{tab:conf_d}
     \end{subtable}
     \hspace*{\fill}
     \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{lrrrr}
        \toprule
          & LOC & ORG & PERS & NA\\
        \midrule    
        LOC & 605 & 18 & 3 & 208\\
        ORG & 141 & 123 & 8 & 536\\
        PERS & 14 & 55 & 826 & 500\\
        NA & 652 & 713 & 388 & 62632\\
        \bottomrule
        \end{tabular}
        \caption{Polyglot}
        \label{tab:conf_p}
     \end{subtable}
     \newline
    \vspace*{0.5 cm}
    \newline
     %\hspace*{\fill}
     \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{lrrrr}
        \toprule
          & LOC & ORG & PERS & NA\\
        \midrule
        LOC & 495 & 34 & 14 & 237\\
        ORG & 657 & 413 & 26 & 3112\\
        PERS & 25 & 103 & 969 & 662\\
        NA & 198 & 383 & 272 & 57875\\
        \bottomrule
        \end{tabular}
        \caption{DaNLP + Polyglot}
        \label{tab:conf_d+p}
    \end{subtable}
    \hspace*{\fill}
    \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{lrrrr}
        \toprule
         & LOC & ORG & PERS & NA\\
        \midrule
        LOC & 722 & 40 & 13 & 295\\
        ORG & 428 & 402 & 20 & 3024\\
        PERS & 27 & 108 & 962 & 610\\
        NA & 233 & 383 & 286 & 60491\\
        \bottomrule
        \end{tabular}
        \caption{Polyglot + DaNLP}
        \label{tab:conf_p+d}
    \end{subtable}

\end{table}

==> Examples/ex_table3.tex <==
\begin{comment}

\begin{table}[!h]
\caption{\label{tab:performance_table}Performance measures for all models. D = DaNLP, P = Polyglot, R = rule based. + indicates multiple taggers used in an ensemble, with the first one being the primary.}
\centering
\begin{tabular}[t]{lllllll}
\toprule
Metric & D + R & D & P & D + P & P + D\\
\midrule
Accuracy & 0.923 & 0.925 & 0.952 & 0.913 & 0.920\\
%acc\_low & 0.921 & 0.923 & 0.950 & 0.910 & 0.918\\
%acc\_high & 0.925 & 0.927 & 0.954 & 0.915 & 0.922\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{LOC}}\\
\hspace{1em}LOC\_F1 & 0.423 & 0.415 & 0.539 & 0.459 & 0.582\\
\hspace{1em}LOC\_Sensitivity & 0.294 & 0.287 & 0.428 & 0.360 & 0.512\\
\hspace{1em}LOC\_Specificity & 0.998 & 0.998 & 0.997 & 0.996 & 0.995\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{PERS}}\\
\hspace{1em}PERS\_F1 & 0.704 & 0.701 & 0.631 & 0.637 & 0.644\\
\hspace{1em}PERS\_Sensitivity & 0.691 & 0.649 & 0.674 & 0.756 & 0.751\\
\hspace{1em}PERS\_Specificity & 0.994 & 0.996 & 0.991 & 0.988 & 0.989\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{ORG}}\\
\hspace{1em}ORG\_F1 & 0.153 & 0.153 & 0.143 & 0.161 & 0.167\\
\hspace{1em}ORG\_Sensitivity & 0.417 & 0.418 & 0.135 & 0.443 & 0.431\\
\hspace{1em}ORG\_Specificity & 0.947 & 0.948 & 0.990 & 0.941 & 0.948\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{Avg}}\\
\hspace{1em}Avg\_F1 & 0.423 & 0.415 & 0.539 & 0.459 & 0.582\\
\hspace{1em}Avg\_Sensitivity & 0.294 & 0.287 & 0.428 & 0.360 & 0.512\\
\hspace{1em}Avg\_Specificity & 0.998 & 0.998 & 0.997 & 0.996 & 0.995\\
\bottomrule
\end{tabular}
\end{table}

\end{comment}


\begin{table}[!h]
\caption{\label{tab:performance_table} Performance measures for all models. D = DaNLP, P = Polyglot, R = rule based. + indicates multiple taggers used in an ensemble with the first one being the primary.}
\centering
\begin{tabular}[t]{lllllll}
\toprule
Metric & D + R & D & P & D + P & P + D\\
\midrule
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{LOC}}\\
\hspace{1em}F1 & 0.423 & 0.415 & 0.539 & 0.459 & 0.582\\
\hspace{1em}Recall & 0.294 & 0.287 & 0.428 & 0.360 & 0.512\\
\hspace{1em}Precision & 0.749 & 0.749 & 0.725 & 0.635 & 0.675\\
\hspace{1em}Specificity & 0.998 & 0.998 & 0.997 & 0.996 & 0.995\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{PERS}}\\
\hspace{1em}F1 & 0.704 & 0.701 & 0.631 & 0.637 & 0.644\\
\hspace{1em}Recall & 0.691 & 0.649 & 0.674 & 0.756 & 0.751\\
\hspace{1em}Precision & 0.718 & 0.763 & 0.592 & 0.551 & 0.564\\
\hspace{1em}Specificity & 0.994 & 0.996 & 0.991 & 0.988 & 0.989\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{ORG}}\\
\hspace{1em}F1 & 0.153 & 0.153 & 0.143 & 0.161 & 0.167\\
\hspace{1em}Recall & 0.417 & 0.418 & 0.135 & 0.443 & 0.431\\
\hspace{1em}Precision & 0.094 & 0.094 & 0.152 & 0.098 & 0.104\\
\hspace{1em}Specificity & 0.947 & 0.948 & 0.990 & 0.941 & 0.948\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{Macro avg.}}\\
\hspace{1em}F1 & 0.423 & 0.415 & 0.539 & 0.459 & 0.582\\
\hspace{1em}Recall & 0.294 & 0.287 & 0.428 & 0.360 & 0.512\\
\hspace{1em}Precision & 0.749 & 0.749 & 0.725 & 0.635 & 0.675\\
\hspace{1em}Specificity & 0.998 & 0.998 & 0.997 & 0.996 & 0.995\\
\bottomrule
\end{tabular}
\end{table}

==> Examples/ex_with_eq.tex <==
%introduction to basics





Let us start off by introducing the activation function of the artificial neurons (henceforth simply neuron). Initial networks used the step function as seen in equation \ref{step}.

\[
s(z)=\begin{cases} 0\quad if\quad z \leq  threshold \\ 1 \quad if\quad z > threshold \end{cases}
\tag{1}
\label{step}
\]

Where $z$ is given by $\sum_i^n w_i x_i+b$, where $x$ is activation of the previous layer and $b$ and $w$ is the bias and weights, while $n$ is the number of neurons in the previous layer. This function follows the conceptual idea that a neuron is either inactive (returns 0) or active (returns 1), however it have the problem of not being differentiable. Consequently we introduce the differentiable sigmoid function, which similar to the step function is a decision function bounded between 0 and 1:

\[
\sigma (z) =  \frac{1}{1+e^{-z}}
\tag{2}
\label{sigmoid}
\]

Notably more recent implementations of \gls{ann}s, such as the Imagenet by \cite{krizhevsky2012imagenet}, have used other activation function such as tanh or reLU which have proved more efficient \citep{krizhevsky2012imagenet}, however the most important feature of the activation function is that it is nonlinear since it then becomes a universal approximator \citep{Kriegeskorte2019}.

For illustrative purposes let us now construct a network consisting of 306 input neurons, two fully connected layers of 32 and 16 neurons and an output layer of 2 neurons, where the input consist of  the 306 MEG channels and their activation 110 seconds after stimulus onset. The two output neurons indicate the two types of stimulus we seek to predict based on the activation. For more on the origin of this data and the nature of the stimuli, see \cite{Kurm2019}\footnote{it is expected that the examiner is familiar with the study}\newline

\begin{figure}
    \caption{A simple \gls{ann} architecture for classifying seen stimulus from MEG signal. The '?' represent a dimension of arbitrary size.}
    \centering
    \includegraphics[width=0.35\textwidth]{pics/simple_nn.png}
    \label{simple_nn}
\end{figure}


\noindent To train this neural network, backpropagation is applied \citep{werbos1974beyond}. This requires a cost function, which should be a differentiable function describing the difference between the desired output and the current output in which completely wrong answer should be attributed a higher cost compared to only a somewhat wrong answer. In this case we will be using the categorical cross entropy cost function which have the desired traits. backpropagation works by calculating the gradient of steepest descent based on the cost function for each layer and the update weight and biases according to the learning rate and the gradient. Conceptually this equates to calculating the direction which would lead to the steepest decrease in cost and then taking a short step equal to a specified rate of learning in the given direction. Due to space limitations this is naturally quite a simplification and in practice several modifications is made e.g. the gradient is only calculated based on a subsection of the training set at a time  (typically referred to as stochastic gradient descent) as it is computationally unfeasable to calculate based on huge samples\footnote{For example Imagenet is trained based on 14 million tagged pictures} and the learning rate varied so that it initially learns fast and then slows down.




==> Examples/ex_with_pics.tex <==
The networks presented is currently only predicting the stimuli using 1 time point and 1 participant and while it obtain good performance it does so with a large degree of overfit compared to alternative models presented by \cite{Kurm2019}. Furthermore \gls{ann} are harder to interpret and more computationally expensive. \footnote{The time used to fit one time point was approximately the time it took to fit a linear SVM to each of 1501 time points.}.

The following tries mend this issue by applying a \gls{rnn} using the \gls{lstm} architecture. The RNN's have been shown to successfully solve sequence related task, such as speech recognition \citep{Srivastava2015}, in which the signal at a given time $t$ is dependent of signal at time $t-1$ which is then dependent on the time before it. Consequently it might be reasonable to expect similar performance when applied to the MEG data, due to its similar structure. The network uses the time points 80-150 seconds after stimulus onset as predictors, as these were found to be the intervals most predictable of facial stimuli in a per participant analysis, furthermore it was trained on all groups, except group 7, with all 306 channels \cite{Kurm2019}. Prior to training both the data was scaled per participant. It should be mentioned that there have been a couple of steps in between the previous fully connected \gls{ann}s and the following RNN have been left out. Naturally these should be seen systematically as to discern the effect of individual changes. Examples include, testing the performance of the dense neural network using multiple participants and predicting a previously unseen participant as well as experimenting with optimization features such as dropout rates.

The architecture of the \gls{rnn} can be seen in figure \ref{lstm_a}. Noticeably the increasing loss on the test set, as seen in figure \ref{lstm_acc} indicate a large degree of overfit with only a slight initial increase in performance, however it should be noted that the model consistently performed slightly above chance level on the test set. However, this is not overly impressive as it seems reasonable to guess that a simpler model, such as a linear SVM, might obtain similar performance without the same degree of overfit.

\begin{figure}
    \caption{The architecture of the best performing network using as LSTM. The '?' represent a dimension of arbitrary size.}
    \centering
    \includegraphics[width=0.80\textwidth]{Examples/lstm_model.png}
    \label{lstm_a}
\end{figure}

\begin{figure}
    \caption{The loss and accuracy of the model shown in figure \ref{lstm_a} }
    \centering
    \includegraphics[width=0.45\textwidth]{Examples/lstm_loss.png}
    \includegraphics[width=0.45\textwidth]{Examples/lstm_acc.png}
    \label{lstm_acc}
\end{figure}


Naturally future studies should cross validate the model rather than simply predicting one participant as done here. Furthermore it might also be interesting to see if image classification on spectrograms of the MEG signal would lead to better performance, as this have shown to be the case for other signal classification tasks \cite{Papakostas2018}.

==> Other/OverviewML.tex <==
ASD (11 studies, up to 2016):
[Santos et al., 2013]: 
    FS: None
    V: 10-fold cross-validation on classifier
    C: probabilistic NN. Accuracy: 83–97%
    C: SVM. Accuracy: 79–63%
[Oller et al., 2010]
    FS: None
    V: Leave-one-out cross-validation
    C: linear DA. Accuracy: 86%
[Bonneh et al., 2011]
    FS: None (2 features only)
    V: None
    C: linear DA Accuracy: 86%
    Sensitivity: 80%
    Specificity: 90%
[Kiss et al., 2012]
    FS: None
    V: Leave-one-out cross-validation
    C: naïve Bayes. Accuracy: 74%
    Precision: 57%
    Sensitivity: 86%
[Kakihara, Takiguchi, Ariki, Nakai, & Takada, 2015]
    FS: None
    V: 10-fold cross-validation
    C: SVM.
    Accuracy: 74.9% (against a baseline accuracy of 73.2%)
[Asgari, Bayestehtashk, & Shafran, 2013]
    FS: None
    V: Test/Train
    C: SVM Sensitivity: 93.80%
[Bone et al., 2013]
[Fusaroli, Bang, & Weed, 2013]
[Fusaroli, Grossman, Cantio, Bilenberg, & Weed, 2015]
[Bone et al., 2014]
[Marchi et al., 2015]

Schizophrenia  (9 studies, up to 2022)
Rapcan et al. (2009)
Martinez-Sanchez et al. (2015)
Kliper et al. (2015) 
Puschel et al. (1998) 
Cohen et al. (2020)
Thair et al. (2019)
Espinola et al., (2021)
de Boer et al., (2022) 
Agurto et al. (2020)

==> Other/github_link.tex <==
\textbf{Github link to source code:} 
https://github.com/KennethEnevoldsen/Placeholder

==> Other/notes_from_thesis.tex <==

Riccardo: 

General comment: we need to streamline: think really hard about the framing, make an outline and subordinate all the details to the main narrative.
 
Introduction: shift to neuropsych conditions (less controversial). Intro on burden of mental disorders is a bit overused in the lit. Maybe we could point straight to the arguments for better assessment. It might make sense to make the lit review on ml models a bit more systematic (Rybner et al has a list of all ml papers on asd, alberto should have another on all for schizo; we could build the one for mdd), in terms of algos and features used, as well as validation procedures, and performance. We need better motivation for using both modalities. An alternative (not sure better, but at least simpler) framing would focus on transformers and keep everything else as backgrounded baseline. 
 
Methods: Chronic MDD is mentioned and I would then ask for how it plays a role. Missing triangle transcriptions can be easily fixed. Untranscribed triangles are easy to fix. The cogsci person me misses a bit more motivation of the different fancy features used: eg are all baseline features of the same kind, or do they cover conceptually different properties of the signal? And how do the transformers differ in terms of the conceptual level properties of the signal? Not necessary if we submit to a ML journal, but definitely if we go into a psych journal. Also we could sum up text and audio baselines in one table. I find the split btw text and audio a bit confusing (too much info to keep track of), maybe draw a general pipeline that applies to both text and voice to help with the overview? We need to comment on the differences in preprocessing (cutting audio vs not cutting text; augmenting audio vs not augmenting text; etc.)
 
Results: generally we need to tell a more linear story with the structure of the results. ? If we do the lit review of previous performance, we want to see how well binomial classifiers compare to the existing literature. n the plots I would also separate vertically baseline, ensemble baseline, transformers, ensemble transformers, to make our progress or lack thereof more explicit. We need to emphasize better the key point that binary classifiers seem high performing and this drops in the multiclass context.Also, how diverse is performance by participant? And by trial within participant? Some of the studies had a fixed order of triangles. It could be interesting to see whether performance is systematically different in the different videos.
 
Discussion: depression has also impaired ToM. We need to open up to more symptom based approaches. Not fully buying the way we push for black boxes (too underargued). Lots of suggestions in the discussion that could actually be performed here.
 

==> Other/outline.tex <==
To do:
- Finalize discussion and add abstract
- Finalize bibliography
- Check internal references (e.g., tables, figures, sections)
- Add affiliations and do some restyling 
- Change labels in figures (ASD, MDD/DEP, SCZ)
- Color code model names in figure 3 (top 10 performance) by modality
- Pipeline figure: 
    - Flip ordering of speech / text (so arrow in the top points left instead of right)
    - Add transformers to the text pipeline
- Move the description of original studies to methods + the diagnostic procedure of the studies
- Søren suggests gathering limitations under a specific heading in the discussion and adding:
    - Arbitrary composition of the groups (e.g. no patients with bipolar, anxiety disorders, personality disorders etc.)
    - Limitations associated with animated triangles task. Other methods of speech elicitation better?
- Convert to word  :'(

Journal:
- Molecular psychiatry
- Schizophrenia bulletin
- Journal of affective disorders

Word length:
- 4-5k words

Framing:
- \textbf{specificity} for clinical/psych audience. Subtheme: more features and fancier models are not gonna solve it, we *also* need more data and more granular meta-data

- Fancier models might overfit more - but also more potential with larger dataset sizes? 

